Token-Level Privacy in Large Language Models

The use of language models as remote services requires transmitting private information to external providers, raising significant privacy concerns. This process not only risks exposing sensitive data to untrusted service providers but also leaves it vulnerable to interception by eavesdroppers. Existing privacy-preserving methods for natural language processing (NLP) interactions primarily rely on semantic similarity, overlooking the role of contextual information. In this work, we introduce dchi-stencil, a novel token-level privacy-preserving mechanism that integrates contextual and semantic information while ensuring strong privacy guarantees under the dchi differential privacy framework, achieving 2epsilon-dchi-privacy. By incorporating both semantic and contextual nuances, dchi-stencil achieves a robust balance between privacy and utility. We evaluate dchi-stencil using state-of-the-art language models and diverse datasets, achieving comparable and even better trade-off between utility and privacy compared to existing methods. This work highlights the potential of dchi-stencil to set a new standard for privacy-preserving NLP in modern, high-risk applications.

==> 9999_attacker.tex <==

\begin{figure*}[t]
    \centering
    \scriptsize
    \begin{tikzpicture}[auto,scale=1.2]
    
        \tikzstyle{embs} = [shape = rectangle, rounded corners]
        
%        \tikzset{>=stealth'}
        \node at (-0.5,4) {Input:};
        \draw [thin, rounded corners] (1,3.75) rectangle (4,4.25);
        \node (input1) at (2.5,4) {what a nice day};
        \draw [thin, rounded corners] (5,3.75) rectangle (8,4.25);
        \node (input2) at (6.5,4) {what what nice unicorn};
        \draw[->]  (input1) edge (input2);

        \node at (-0.5,1){Attacker path:};
        
        
        \draw [thin, rounded corners,fill=green!30] (0.5,1.75) rectangle (1.5,2.25);
        \node (awprob) at (1,2.4) {$p=80\%$};
         \node (w) at (1,2) {what};
         \draw [thin, rounded corners,fill=green!30] (0.5,-0.25) rectangle (1.5,0.25);
         \node (aprob) at (1,0.4) {$p=20\%$};
         \node (a) at (1,0) {a};

         \draw [thin, rounded corners,fill=red!30] (2, 2.25) rectangle (3.5, 2.75);
         \node (ww) at (2.75,2.5) {what what};
         \node (wwprob) at (2.75,2.9) {$p=80\% \times 0.1\%$};
         \draw [thin, rounded corners,fill=green!30] (2, 1.25) rectangle (3.5, 1.75);
         \node (wa) at (2.75,1.5) {what a};
         \node (waprob) at (2.75,1.9) {$p=80\% \times 99.9\%$};
         \draw[->]  (w) edge (2,2.5);
         \draw[->]  (w) edge (2,1.5);

         \draw [thin, rounded corners,fill=red!30] (2, 0.25) rectangle (3.5, 0.75);
         \node (aw) at (2.75,0.5) {a what};
         \node (awprob) at (2.75,0.9) {$p=20\% \times 10\%$};
         \draw [thin, rounded corners,fill=green!30] (2, -0.75) rectangle (3.5, -0.25);
         \node (aa) at (2.75,-0.5) {a a};
         \node (aaprob) at (2.75,-0.1) {$p=20\% \times 90\%$};
         \draw[->]  (a) edge (2, 0.5);
         \draw[->]  (a) edge (2, -0.5);

%% 3rd lvl
        \draw [thin, rounded corners,fill=green!30] (4.25, 2.25) rectangle (6.25, 2.75);
         \node (wab) at (5.25,2.5) {what a nice};
        \node (wwprob) at (5.25,2.9) {$p=80\% \times 99.9\% \times 90\%$};
         \draw [thin, rounded corners,fill=red!30] (4.25, 1.25) rectangle (6.25, 1.75);
         \node (wad) at (5.25,1.5) {what a is};
        \node (waprob) at (5.25,1.9) {$p=80\% \times 99.9\% \times 10\%$};
         \draw[->]  (3.3,1.6) -> (4.25,2.5);
         \draw[->]  (3.3,1.5) -> (4.25,1.5);


       \draw [thin, rounded corners,fill=green!30] (4.25, 0.25) rectangle (6.25, 0.75);
         \node (aab) at (5.25, 0.5) {a a nice};
         \node (wwprob) at (5.25,0.9) {$p=20\% \times 90\% \times 90\%$};
         \draw [thin, rounded corners,fill=red!30] (4.25, -0.75) rectangle (6.25, -0.25);
         \node (aad) at (5.25,-0.5) {a a is};
        \node (waprob) at (5.25,-0.1) {$p=20\% \times 90\% \times 10\%$};
         \draw[->]  (3.3,-0.4) -> (4.25,0.5);
         \draw[->]  (3.3,-0.5) -> (4.25,-0.5);
        
%% 4th lvl
        \draw [thin, rounded corners] (7, 2.25) rectangle (10, 2.75);
         \node (wab) at (8.5,2.5) {what a nice unicorn};
         \node (wwprob) at (8.5,2.9) {$p=80\% \times 99.9\% \times 90\% \times 1\%$};
         \node (wwprob) at (11,2.5) {$P=7.1928\%$};
         \draw [thin, rounded corners,fill=green!100] (7, 1.25) rectangle (10, 1.75);
         \node (wad) at (8.5,1.5) {what a nice day};
         \node (wwprob) at (11,1.5) {\textbf{$P=64.7352\%$}};
        \node (waprob) at (8.5,1.9) {$p=80\% \times 99.9\% \times 90\% \times99\%$};
         \draw[->]  (6.3,2.5) -> (7,2.5);
         \draw[->]  (6.3,2.3) -> (7,1.5);

       \draw [thin, rounded corners] (7, 0.25) rectangle (10, 0.75);
         \node (aab) at (8.5, 0.5) {a a nice day};
         \node (wwprob) at (8.5,0.9) {$p=20\% \times 90\% \times 90\% \times 50\%$};
         \node (wwprob) at (11,0.5) {$P=8.1\%$};

         \draw [thin, rounded corners] (7, -0.75) rectangle (10, -0.25);
         \node (aad) at (8.5,-0.5) {a a is unicorn};
         \node (waprob) at (8.5,-0.1) {$p=20\% \times 90\% \times 90\% \times 50\%$};
         \node (wwprob) at (11,-0.5) {$P=8.1\%$};
         \draw[->]  (6.3,0.5) -> (7,0.5);
         \draw[->]  (6.3,0.3) -> (7,-0.5);

    
        
        
        
    
    \end{tikzpicture}
    
    \caption{Schematic overview of the proposed heuristic oracle attacking scenario path over trying to reconstruct the sentence ``what a nice day'' which is remapped to ``what what nice unicorn''. 
    The red boxes indicate that the probability (presented above the box) of the candidate is low enough to be dropped in the next step, while the green boxes are the candidates that will be expanded in the next step.}
    \label{fig:attacker}
\end{figure*}


==> 9999_framework.tex <==
\begin{figure}[t]
    \centering
    \scriptsize
    \begin{tikzpicture}[auto, scale=0.7]
    
        \tikzstyle{embs} = [shape = rectangle, rounded corners]
        
%        \tikzset{>=stealth'}
        
        % \node at (8.5,-5.75) {Input};
        \draw [thin, rounded corners] (0.5,-4.75) rectangle (2.5,-5.25);
        \node (input) at (1.5,-5) {Input data};

        \draw[line width=0.75mm, draw=black!55, dashed] (-5,-4.5) -- (5,-4.5);
        \node[text width=9cm] at (0.75,-4.25) {(A) Text privatization};

        \draw [fill=archtBlue, thin, double, rounded corners] (0,-3.75) rectangle (3,-4.25);
         \node at (1.5,-4) {Tokenizer};

        \draw[->] (input) edge (1.5,-4.25);
        %% TOKENS
        \draw [thin,fill=archtBlue!40, rounded corners] (-0.8,-2.75) rectangle (0.3,-3.25);
        \draw [thin,fill=archtBlue!40, rounded corners] (0.55,-2.75) rectangle (1.65,-3.25);
        \draw [thin,fill=archtBlue!40, rounded corners] (1.8,-2.75) rectangle (2.9,-3.25);
        \draw [thin,fill=archtBlue!40, rounded corners] (3.15,-2.75) rectangle (4.25,-3.25);
        \node (t3) at (-0.25,-3) {Token$_1$};
        \node (t4) at (1.1,-3) {Token$_2$};
        \node (t5) at (2.4,-3) {Token$_3$};
        \node (t6) at (3.7,-3) {Token$_4$};
        
        \draw[->]  (1.5,-3.75) edge (t3.south);
        \draw[->]  (1.5,-3.75) edge (t4.south);
        \draw[->]  (1.5,-3.75) edge (t5.south);
        \draw[->]  (1.5,-3.75) edge (t6.south);


        \draw[->]  (t3) edge (-0.25,-2.25);
        \draw[->]  (t4) edge (1.1,-2.25);
        \draw[->]  (t5) edge (2.4,-2.25);
        \draw[->]  (t6) edge (3.7,-2.25);
        
        \draw [fill=archtOrange, thin, double, rounded corners] (-1.25,-2.25) rectangle (4.6,-1.75) ;
        \node at (1.5, -2.05) {Embedding table};
        \draw[line width=0.75mm, draw=blue!55, dashed] (-5,-2.5) -- (5,-2.5);
        \node[text width=9cm] at (0.75,-2.2) {(B) Token privatization};

        
   
        \draw[<-]  (-0.25,-1.25) edge (-0.25,-1.75);
        \draw[<-]  (1.1,-1.25) edge (1.1 ,-1.75);
        \draw[<-]  (2.4,-1.25) edge (2.4,-1.75);
        \draw[<-]  (3.7,-1.25) edge (3.7,-1.75);
        
        \draw [thin, rounded corners, fill=yellow!25] (-0.85,-0.85) rectangle (0.35,-1.25);
              \node [matrix] (e3) at (-0.25,-1.05) {
              \draw [fill=orange!55] circle (0.75mm); & \draw [fill=orange!55] circle (0.75mm); & \draw [fill=orange!55] circle (0.75mm); & \draw [fill=orange!55] circle (0.75mm);  \\
              };
        \draw [thin, rounded corners, fill=yellow!25] (0.45,-0.85) rectangle (1.65,-1.25);
              \node [matrix] (e4) at (1.05,-1.05) {
              \draw [fill=orange!55] circle (0.75mm); & \draw [fill=orange!55] circle (0.75mm); & \draw [fill=orange!55] circle (0.75mm); & \draw [fill=orange!55] circle (0.75mm);  \\
              };
        \draw [thin, rounded corners, fill=yellow!25] (1.75,-0.85) rectangle (2.95,-1.25);
              \node [matrix] (e5) at (2.35,-1.05) {
              \draw [fill=orange!55] circle (0.75mm); & \draw [fill=orange!55] circle (0.75mm); & \draw [fill=orange!55] circle (0.75mm); & \draw [fill=orange!55] circle (0.75mm);  \\
              };
        \draw [thin, rounded corners, fill=yellow!25] (3.05,-0.85) rectangle (4.25,-1.25);
              \node [matrix] (e6) at (3.65,-1.05) {
              \draw [fill=orange!55] circle (0.75mm); & \draw [fill=orange!55] circle (0.75mm); & \draw [fill=orange!55] circle (0.75mm); & \draw [fill=orange!55] circle (0.75mm);  \\
              };
        \draw[line width=0.75mm, draw=red!55, dashed] (-5,-0.6) -- (5,-0.6);
        \node[text width=9cm] at (0.75,-0.35) {(C) Token embedding privatization};

      \draw [fill=green!25, thin, double, rounded corners] (-1.25,-0.15) rectangle (4.6,0.35) ;
        \node at (1.5, 0.1) {Encoder};

        \draw[->]  (e3) edge (1.675,-0.15);
        \draw[->]  (e4) edge (1.675,-0.15);
        \draw[->]  (e5) edge (1.675,-0.15);
        \draw[->]  (e6) edge (1.675,-0.15);
        
        \draw [thin, rounded corners, fill=green!25] (-0.85,0.7) rectangle (0.35,1.1);
              \node [matrix] (o3) at (-0.25,0.9) {
              \draw [fill=green] circle (0.75mm); & \draw [fill=green] circle (0.75mm); & \draw [fill=green] circle (0.75mm); & \draw [fill=green] circle (0.75mm);  \\
              };
        \draw [thin, rounded corners, fill=green!25] (0.45,0.7) rectangle (1.65,1.1);
              \node [matrix] (o4) at (1.05,0.9) {
              \draw [fill=green] circle (0.75mm); & \draw [fill=green] circle (0.75mm); & \draw [fill=green] circle (0.75mm); & \draw [fill=green] circle (0.75mm);  \\
              };
        \draw [thin, rounded corners, fill=green!25] (1.75,0.7) rectangle (2.95,1.1);
              \node [matrix] (o5) at (2.35,0.9) {
              \draw [fill=green] circle (0.75mm); & \draw [fill=green] circle (0.75mm); & \draw [fill=green] circle (0.75mm); & \draw [fill=green!55] circle (0.75mm);  \\
              };
        \draw [thin, rounded corners, fill=green!25] (3.05,0.7) rectangle (4.25,1.1);
              \node [matrix] (o6) at (3.65,0.9) {
              \draw [fill=green] circle (0.75mm); & \draw [fill=green] circle (0.75mm); & \draw [fill=green] circle (0.75mm); & \draw [fill=green] circle (0.75mm);  \\
              };
              
 
        \draw[->] (1.675,0.35) -> (o3);
        \draw[->] (1.675,0.35) -> (o4);
        \draw[->] (1.675,0.35) -> (o5);
        \draw[->] (1.675,0.35) -> (o6);

    \draw[line width=0.75mm, draw=green!55, dashed] (-5,1.3) -- (5,1.3);
    \node[text width=9cm] at (0.75,1.6) {(D) Sequence embedding privatization};


    
    \end{tikzpicture}
    
    \caption{A schematic of the various stages where differential privacy techniques can be applied in an LLM. This work focuses on level (B).}
    \label{fig:pipeline}
\end{figure}


==> figures/qwen_figure.tex <==
\begin{figure*}[ht]
    \centering
     %\begin{subfigure}[t]{0.45\textwidth}
     \includegraphics[width=0.47\linewidth]{figures/qwen_swag.pdf}
     \includegraphics[width=0.47\linewidth]{figures/qwen_mmlu.pdf}
     \\
     \includegraphics[width=0.97\linewidth]{figures/qwen_legend.pdf}
    %\includegraphics[width=0.5\linewidth]{}
    \caption{The affect of $\sigma$, $\eta$ and $\epsilon$ on the accuracy and Pr@5 for the \econvdef{} and \custext{} methods. 
    The left graph presents the results of \flan{} over the QNLI dataset, while the right graph presents the results of \qwen{} over the SWAG dataset.
    The Clean trend exhibits the baseline of the unsanitized data.}
    \label{fig:ablation}
\end{figure*}

==> latex_tips.tex <==

\uvp{\small
Some of my \LaTeX{} rules:
Full parenthetical citations (\texttt{\textbackslash{}cite} or \texttt{\textbackslash{}citep}) are preceded by a NBSP (tilde).
Each sentence gets its own source line (so it can be easily found, moved around, commented out).
We use \say{\texttt{\textbackslash{}say}} for quotes.
We don't use \texttt{\textbackslash{}subsubsections}---stuff below \texttt{\textbackslash{}subsection} gets \texttt{\textbackslash{}paragraph}.
We don't use \texttt{\textbackslash{}vspace} and its friends, definitely not in drafts.
When we have enough prose in a section (or sooner, whatever's convenient), we extract it to its own file.
\url{http://detexify.kirelabs.org/classify.html} is a life-saver.
We use macros for names and terms that might change, like system names, and for inconveniently long but often-used phrases.
Numbers in the body of the text don't get put in mathmode.
Tables: no vertical lines, ever.
Minimal horizontal lines, using the \texttt{\textbackslash{}booktabs} extension (toprule and bottomrule in borders, midrule below legend and between coarse-grain row groups).
Anything that was published in a peer-reviewed venue is cited by its published venue, not arXiv.
If it was in an ACL-indexed venue, all you have to do is look it up on the anthology website (I have a Chrome shortcut for anthology search) and single-click-copy the bibkey, since we have the bib file already. Example:~\cite{klymenko-etal-2022-differential}.
For more: \href{https://medium.com/@vered1986/tips-for-writing-nlp-papers-9c729a2f9e1f}{here.}}


==> tables/9_ablation.tex <==
% \begin{figure*}[ht]
%     \centering
%     % First plot
%     \begin{subfigure}[t]{0.45\textwidth}
%         \centering
%         \begin{tikzpicture}
%             \begin{axis}[
%                 xlabel={Pr@5 (lower better)},
%         ylabel={Accuracy (higher better)},
%          title={\flan{} on QNLI},
%         xmin=0.4, xmax=1.02,
%          width=\textwidth,
%         ymin=0.5, ymax=0.91,
%        legend to name={mylegend},
%         grid=both,
%        legend style={at={(0.5,-0.2)}, anchor=south, legend columns=-1}
%             ]

%             % sigma 0.5, t5 qnli
%             \addplot[
%             thick,
%             mark=*,
%             color=blue,
%             mark options={fill=blue},
%             nodes near coords,
%             point meta=explicit symbolic,
%             every node near coord/.append style={anchor=south, yshift=3pt}
%         ] coordinates {
%             (0.52695, 0.6694) [\footnotesize $\eta=175$]
%             (0.57484, 0.6972) [\footnotesize $\eta=200$]
%             (0.62765, 0.7274) [\footnotesize $\eta=250$]
%             (0.65443, 0.7445) [\footnotesize $\eta=300$]
%             (0.69217, 0.7595) [\footnotesize $\eta=350$]
%             (0.70445, 0.7755) [\footnotesize $\eta=1000$]
%         };

%         % sigma 0.7, t5 qnli
%         \addplot[
%             thick,
%             mark=square*,
%             color=red,
%             mark options={fill=red},
%             nodes near coords,
%             point meta=explicit symbolic,
%         every node near coord/.append style={anchor=north, yshift=-2pt, xshift=3pt}
%         ] coordinates {
%             (0.44428, 0.6006) [\footnotesize $\eta=175$]
%             (0.49992, 0.6266) [\footnotesize $\eta=200$]
%             (0.57628, 0.6786) [\footnotesize $\eta=250$]
%             (0.61815, 0.7049) [\footnotesize $\eta=300$]
%             (0.64326, 0.7271) [\footnotesize $\eta=350$]
%             (0.69907, 0.7696) [\footnotesize $\eta=1000$]
%         };

%         % sigma 1.0, t5 qnli
%         \addplot[
%             thick,
%             mark=triangle*,
%             color=mGreen,
%             mark options={fill=mGreen},
%             nodes near coords,
%             point meta=explicit symbolic,
%             every node near coord/.append style={anchor=north, yshift=-2pt, xshift=2pt}
%         ] coordinates {
%             (0.40839, 0.5707) [\footnotesize $\eta=175$]
%             (0.47203, 0.5832) [\footnotesize $\eta=200$]
%             (0.55849, 0.6163) [\footnotesize $\eta=250$]
%             (0.60964, 0.6442) [\footnotesize $\eta=300$]
%             (0.64212, 0.6723) [\footnotesize $\eta=350$]
%             (0.70053, 0.7324) [\footnotesize $\eta=1000$]
%         };
        
%        % custext t5 qnli
%         \addplot[
%             thick,
%             mark=star,
%             color=purple,
%             mark options={fill=purple},
%             nodes near coords,
%             point meta=explicit symbolic,
%             every node near coord/.append style={anchor=north, yshift=-3pt, xshift=8pt}
%         ] coordinates {
%             (0.59662, 0.62) [\footnotesize $\epsilon=3$]
%             (0.68079, 0.6674) [\footnotesize $\epsilon=5$]
%             (0.73271, 0.6857) [\footnotesize $\epsilon=6$]
%             (0.81089, 0.7472) [\footnotesize $\epsilon=7.5$]
%             (0.87734, 0.7975) [\footnotesize $\epsilon=9$]
%         };
%     % clean t5 qnli
%         \addplot[
%             thick,
%             mark=dashed,
%             dashed,
%             color=black,
%             mark options={fill=black},
%             nodes near coords,
%             point meta=explicit symbolic,
%             every node near coord/.append style={anchor=north, yshift=-6pt, xshift=1pt}
%         ] coordinates {
%             (0.0, 0.904) 
%             (0.7, 0.904) [\small Clean]
%             (1.0, 0.904)
%             (1.0, 0.0)
%         };
%                 \legend{\econvdef{}($\sigma=0.5$), \econvdef{}($\sigma=0.7$), \econvdef{}($\sigma=1.0$), Custext, Clean};

%             \end{axis}
%         \end{tikzpicture}

%     \end{subfigure}
%     \hfill
%     % Second plot
%     \begin{subfigure}[t]{0.45\textwidth}
%         \centering
%         \begin{tikzpicture}
%             \begin{axis}[
%           xlabel={Pr@5 (lower better)},
%         ylabel={Accuracy (higher better)},
%         xmin=0.4, xmax=1.02,
%         ymin=0.33, ymax=0.53,
%          width=\textwidth,
%          title={\qwen{} on SWAG},
%         grid=both
%             ]
                
%             % sigma 0.5 qwen2 swag
%      \addplot[
%             thick,
%             mark=*,
%             color=blue,
%             mark options={fill=blue},
%             nodes near coords,
%             point meta=explicit symbolic,
%             every node near coord/.append style={anchor=south, yshift=3pt}
%         ] coordinates {
%             (0.46369, 0.4212) [\footnotesize $\eta=175$]
%             (0.50649, 0.4328) [\footnotesize $\eta=200$]
%             (0.55699, 0.4445) [\footnotesize $\eta=250$]
%             (0.58117, 0.4479) [\footnotesize $\eta=300$]
%             (0.59541, 0.4522) [\footnotesize $\eta=350$]
%             (0.62542, 0.4634) [\footnotesize $\eta=1000$]
%         };

%     % sigma 0.7 qwen2 swag
%         \addplot[
%             thick,
%             mark=square*,
%             color=red,
%             mark options={fill=red},
%             nodes near coords,
%             point meta=explicit symbolic,
%         every node near coord/.append style={anchor=north, yshift=-2pt, xshift=3pt}
%         ] coordinates {
%             (0.37375, 0.3607) [\footnotesize $\eta=175$]
%             (0.42866, 0.3948) [\footnotesize $\eta=200$]
%             (0.49797, 0.4138) [\footnotesize $\eta=250$]
%             (0.53261, 0.4237) [\footnotesize $\eta=300$]
%             (0.55286, 0.4309) [\footnotesize $\eta=350$]
%             (0.59752, 0.4499) [\footnotesize $\eta=1000$]
%         };

%         % sigma 1.0 qwen2 swag
%         \addplot[
%             thick,
%             mark=triangle*,
%             color=mGreen,
%             mark options={fill=mGreen},
%             nodes near coords,
%             point meta=explicit symbolic,
%             every node near coord/.append style={anchor=north, yshift=-6pt, xshift=5pt}
%         ] coordinates {
%             (0.3528, 0.3693) [\footnotesize $\eta=175$]
%             (0.40978, 0.3753) [\footnotesize $\eta=200$]
%             (0.48576, 0.3869) [\footnotesize $\eta=250$]
%             (0.52676, 0.3956) [\footnotesize $\eta=300$]
%             (0.55024, 0.4025) [\footnotesize $\eta=350$]
%             (0.58989, 0.4081) [\footnotesize $\eta=1000$]
%         };
        
% % custext qwen2 swag
%         \addplot[
%             thick,
%             mark=star,
%             color=purple,
%             mark options={fill=purple},
%             nodes near coords,
%             point meta=explicit symbolic,
%             every node near coord/.append style={anchor=north, yshift=-3pt, xshift=4pt}
%         ] coordinates {
%             (0.50787, 0.3994) [\footnotesize $\epsilon=3$]
%             (0.63134, 0.4231) [\footnotesize $\epsilon=5$]
%             (0.70105, 0.4388) [\footnotesize $\epsilon=6$]
%             (0.79633, 0.4642) [\footnotesize $\epsilon=7.5$]
%             (0.8742, 0.4834) [\footnotesize $\epsilon=9$]
%         };
    
%         % clean qwen2 swag
%         \addplot[
%             thick,
%             mark=dashed,
%             dashed,
%             color=black,
%             mark options={fill=black},
%             nodes near coords,
%             point meta=explicit symbolic,
%             every node near coord/.append style={anchor=north, yshift=-4pt, xshift=1pt}
%         ] coordinates {
%             (0.0, 0.52) 
%             (0.75, 0.52) [\small Clean]
%             (1.0, 0.52) 
%             (1.0, 0.0) 
%         };
%             \end{axis}

%         \end{tikzpicture}
%         %\caption{Ablation study of various $\sigma$ sizes of the stencilNoise method with a fixed window size of 15 on the SWAG benchmark, with Qwen2 model effect on the accuracy and Pr@5.}
        
%     \end{subfigure}
   
    
%    {\black\ref{mylegend}}
   
%     \caption{The affect of $\sigma$, $\eta$ and $\epsilon$ on the accuracy and Pr@5 for the \econvdef{} and \custext{} methods. 
%     The left graph presents the results of \flan{} over the QNLI dataset, while the right graph presents the results of \qwen{} over the SWAG dataset.
%     The Clean trend exhibits the baseline of the unsanitized data.
%     }
%     \label{fig:side-by-side}
% \end{figure*}

==> tables/9_ablation2.tex <==
\begin{figure*}[ht]
    \centering
     %\begin{subfigure}[t]{0.45\textwidth}
     \includegraphics[width=0.47\linewidth]{figures/output-figure0.pdf}
     \includegraphics[width=0.47\linewidth]{figures/output-figure1.pdf}
     \\
     \includegraphics[]{figures/output-figure_crossref0.pdf}
    %\includegraphics[width=0.5\linewidth]{}
    \caption{The affect of $\sigma$, $\eta$ and $\epsilon$ on the accuracy and Pr@5 for the \econvdef{} and \custext{} methods. 
    The left graph presents the results of \flan{} over the QNLI dataset, while the right graph presents the results of \qwen{} over the SWAG dataset.
    The Clean trend exhibits the baseline of the unsanitized data.}
    \label{fig:ablation}
\end{figure*}

==> tables/9_final_results.tex <==
\begin{table*}
\centering
\begin{tabular}{llccr }

\toprule
%&  & \multicolumn{2}{c}{\textbf{\flan{}}}&  \multicolumn{2}{c}{\textbf{\qwen{}}}\\
  
  \textbf{Dataset} & \textbf{Method}  & \textbf{\flan{} ($\uparrow$)}  & \textbf{\qwen{} ($\uparrow$)}&  \textbf{Pr@5 ($\downarrow$)}\\ \midrule


SST-2 & Clean & 94.50 & 91.30  &  ---\\
& \econvdef{}$(L=5,\sigma=0.75, \eta=175)$ & 88.30 & 82.00 & 71.83 \\
& \econvdef{}$(L=4,\sigma=0.75, \eta=210)$ & 84.86 & 79.24 & 52.07 \\
& \convdef{}$(L=5,\sigma=1.25)$ & 84.75  & 77.75 & 70.01  \\
& \noise{}$(\eta=100)$  & 87.61 & 82.34 & 72.93 \\
& \custext{}$(\epsilon=7.5)$  & 88.07 & 80.62 &  72.54 \\
\midrule	


QNLI & Clean & 90.04  & --- & --- \\
& \econvdef{}$(L=9,\sigma=0.75, \eta=175)$ & 80.08 & --- & 80.78 \\
& \econvdef{}$(L=8,\sigma=0.75, \eta=250)$ & 78.49 & --- & 62.58 \\
& \convdef{}$(L=5,\sigma=1.25)$ & 80.78  & --- & 81.05  \\
& \noise{}$(\eta=100)$  & 80.08 & ---  & 84.30 \\
& \custext{}$(\epsilon=9)$  & 79.74 & --- & 83.40 \\
\midrule

SWAG & Clean & 47.77 & 52.60  & ---  \\
& \econvdef{}$(L=9,\sigma=0.5, \eta=120)$ & 42.57 & 46.31 & 73.77 \\
& \econvdef{}$(L=6,\sigma=0.75, \eta=210)$ & 40.52 & 44.84 & 55.65 \\
& \convdef{}$(L=5,\sigma=1.25)$ & 40.74  & 45.02 & 79.82  \\
& \noise{}$(\eta=100)$  & 42.97 & 46.59  & 75.23 \\
& \custext{}$(\epsilon=7.5)$  & 42.51 & 46.42 & 73.74 \\
\midrule

MMLU & Clean & 41.54 & 60.43  & ---  \\
& \econvdef{}$(L=9,\sigma=0.75, \eta=160)$ & 38.40 & 54.32 & 74.58 \\
& \econvdef{}$(L=6,\sigma=0.75, \eta=210)$ & 37.46 & 53.47 & 59.12 \\
& \convdef{}$(L=5,\sigma=1.25)$ & 37.81  & 53.50 & 71.33  \\
& \noise{}$(\eta=100)$  & 38.65 & 54.59  & 79.05 \\
& \custext{}$(\epsilon=7.5)$  & 38.11 & 53.36 & 76.73 \\

% MMLU & Clean & 41.39  & A &--- \\
% & \convdef{} & 0 & 0 & A \\
% %& \pconvdef{} & 0 & 0 & A & B\\
%  & \econvdef{}  & 33.99 & 49.81 & A \\
% %& \noise{}($\eta=100)$  & A & B & A & B\\
% & \custext{}  & 34.25 & 97.82 & A \\





\bottomrule
\end{tabular}
\caption{Utility-privacy trade-off comparison between the privatization techniques: \convdef{}, \econvdef{} and \custext{}, over the performance of \flan{} and \qwen{} on the SST-2, QNLI, MMLU and SWAG datasets. 
}
\label{table:final_results}
\end{table*}

==> tables/oovs.tex <==
\begin{table}
\centering
\small
\begin{tabular}{lrrr}
\toprule
\textbf{Dataset} & \textbf{Avg tokens} &\textbf{Total tokens} & \textbf{OOVs} \\
\midrule
SST-2 & 19.5 &17,046 & 129 \\%& 0.75\%  \\
QNLI  & 37.5 &205,581 & 24,392 \\%& 11.86\%  \\
SWAG  & 14.5 &291,311 & 18,005 \\%& 6.18\%  \\
MMLU  & 46.6 & 71,782s &  \\%& A\%  \\
%BBH   & 415,777 & 83,451 & 4.98\%  \\
%MUSR  & 551,077 & 75,022 & 7.34\% \\

\bottomrule
\end{tabular}
\caption{Statistical details of the average tokens per instance and OOVs in each of the experimental datasets.}
\label{table:oovs}
\end{table}
